An EEG-Based Multi-Modal Emotion Database with Both Posed and Authentic Facial Actions for Emotion Analysis

Emotion is an experience associated with a particular pattern of physiological activity along with different physiological, behavioral and cognitive changes. One behavioral change is facial expression, which has been studied extensively over the past few decades. Facial behavior varies with a person's emotion according to differences in terms of culture, personality, age, context, and environment. In recent years, physiological activities have been used to study emotional responses. A typical signal is the electroencephalogram (EEG), which measures brain activity. Most of existing EEG-based emotion analysis has overlooked the role of facial expression changes. There exits little research on the relationship between facial behavior and brain signals due to the lack of dataset measuring both EEG and facial action signals simultaneously. To address this problem, we propose to develop a new database by collecting facial expressions, action units, and EEGs simultaneously. We recorded the EEGs and face videos of both posed facial actions and spontaneous expressions from 29 participants with different ages, genders, ethnic backgrounds. Differing from existing approaches, we designed a protocol to capture the EEG signals by evoking participants' individual action units explicitly. We also investigated the relation between the EEG signals and facial action units. As a baseline, the database has been evaluated through the experiments on both posed and spontaneous emotion recognition with images alone, EEG alone, and EEG fused with images, respectively. The database will be released to the research community to advance the state of the art for automatic emotion recognition.

==> rebuttal.tex <==
Our rebuttal:

Reviewer #1:

Q1: It’s a good idea to random the order of tasks during the data collection period to avoid some negative effects on the experiment. However, before the formal experiment, we collected 7 test shots from 7 participants, and we find that the quality of data we collect is not dependent on the order of the tasks. After analyzing these test shots, we find that it’s highly dependent on whether the participants are or are not good at the task. For instance, some participants can not finish action unit 2(outer brow raiser on one side), no matter what order it is and how we train the participant. Therefore, randomizing the order of the tasks is not in our consideration.

Q2: Yes. Participants manually rate the physical pain level from 0 to 10, where 0 means no-pain and 10 means the worst possible pain. Considering this subjective rating method, the self-reports are used to be the reference to label the data.
Q3: System synchronization is a critical process for data collection from multi-modality sensors. Both of the EEG recording system and video recording software can generate timestamp when starting and ending the recording process. By comparing and calculating the timestamps of starting time from different sensors, we can obtain an accurate synchronized signal.

Q4: STD means standard deviation in this paper. In Table IV, we show the standard deviations of the average accuracies of all cross folds by using different models. We will add the corresponding explanation of the abbreviation to the table description in the revised version.

Q5: Yes, it’s a good suggestion to let the table have more visualized information. We will add the color map to the confusion matrix in the revised version. 


Reviewer #2:

Q1: Yes. During the annotation stage, annotators labeled the dataset separately and compared these annotations to conclude the quality of the annotation. All of the annotators make the annotations independently and reach a high inter-annotator agreement.

Q2: Fig-6 shows the Feature-C, instead of Feature-A. We’re sorry for making such mistakes, and we will correct it in our latter version.
Q3: The convolutional neural network (CNN) can learn higher level features from training data. When EEG signal is represented visually as a spectrogram, CNNs can also be applied to it. It’s quite similar to the sound signal. Some works have already applied CNN on EEG signals successfully: [1]Vrbancic G and Podgorelec V 2018 Automatic classification of motor impairment neural disorders from EEG signals using deep convolutional neural networks Elektron. Elektrotech. 24 3–7; [2]Kuanar S, Athitsos V, Pradhan N, Mishra A and Rao K R Cognitive analysis of working memory load from EEG, by a deep recurrent neural network 2018 IEEE Int. Conf. on Acoustics, Speech and Signal Processing (ICASSP) pp 352–5. We agree with that facial pose normalization could help for facial action recognition in the most dataset of spontaneous facial action analysis. However, we didn’t apply facial pose normalization, because most of the tasks we did are based on the facial expression imitation and the participants don’t have obvious pose variance like other interview-based experiments.
Q4: This paper does not address how we arrange and train the DANN. Some current works have present the architecture of DANN and training details and tricks well. Please refer to the papers: [1] Y. Ganin et al. Domain-adversarial training of neural networks. Advances in Computer Vision and Pattern Recognition, 2017. [2]H. Li, B.-L. Lu, et al. Cross-subject emotion recognition using deep adaptation networks. In Neural Information Processing. 2018. However, if needed, we can provide the architecture and specification of DANN in the supplementary material. We can also make the source code public so that it can help others’ validation experiments.


Reviewer #3:
To justify that there is no bias picked based on gender or ethnicity in our data set, we split our data set into 2 parts: one contains 15 asian males subject for training, the other one contains other subjects for testing. We get the comparison result of single modal features and fusion features for posed expression recognition using DANN. The reviewer can compare it with the results in Table IV of the paper. The accuracy is: EEG Feature A 75.05%, EEG Feature B 67.23%, EEG Feature C 63.42%, Facial expression image 47.25%, Fusion Feature A 76.42%, Fusion Feature B 59.73%, Fusion Feature C 69.77%.
We find the additional result is basically consistent with the results in Table IV. Fusion features get better performance roughly and the absolute value of  top accuracy 76.42% has negligible gap with the result 76.68% in 4 fold cross validation. Therefore, we believe  there is no bias picked based on gender or ethnicity in our data set.
However, it’s interesting that we find an obvious accuracy reduction using facial expression image feature. 47.25% accuracy is not only lower than the features from other modality, but also lower than the results in table IV. Does it mean that visual modal data are more sensitive to the subject's gender and ethnicity? Or does the EEG signal have universal representation in facial expression recognition across different gender and ethnicity. It’s a very interesting topic. Anyway, before giving a solid conclusion, we still need sufficient experiments to explore it in our future work.

